Using The Concept Hierarchy for Household Action Recognition

We propose a method to systematically represent both the static and the dynamic components of environments, i.e. objects and agents, as well as the changes that are happening in the environment, i.e. the actions and skills performed by agents. Our approach, the Concept Hierarchy, provides the necessary information for autonomous systems to represent environment states, perform action modeling and recognition, and plan the execution of tasks. Additionally, the hierarchical structure supports generalization and knowledge transfer to environments. We rigorously define tasks, actions, skills, and affordances that enable human-understandable action and skill recognition.

==> ch2_related_work.tex <==
\section{Related Work}
\todo{Add related work}


\commenting{
\noindent\textbf{Learning by Watching. }Allowing constrained task execution and generalization to various scenarios by emulating human demonstrations has been a long-time goal of the scientific community. 
The seminal work 
% In 1990, 
\cite{teachingByShowing} introduced the term \textit{teaching by showing}, followed by \cite{learningByWatchingFirst} which designed a \textit{Learning by Watching} (LbW) system which was used to represent a task plan and generalize it to a new environment. LbW~\cite{yu2018one, liu2018imitation} in comparison to other paradigms, doesn't rely on kinesthetic or robot demonstrations thereby providing a more intuitive interface. Since then, a plethora of imitation models have been explored~\cite{smith2019avid, shao2021concept2robot, sermanet2018time, wang2019learning, brandi2014generalizing, wang2020see, jin2020geometric}. 
In this context, \cite{taskLearningByWatching} uses a single video demonstration and a learning-by-watching paradigm to perform action-imitation that can generalize to a different kinematic structure.~\cite{li2021meta} goes a step further and presents a meta learning algorithm that is able to learn new tasks by watching only a single video, although they use a great number of demonstrations  during training in simulation. A manipulation policy using pose retargeting (to different robotic hands) after the initial acquisition of RGBD data from human demonstration is presented in~\cite{qin2022one}. \cite{bahl2022human} proposes a one-shot learning algorithm that takes in extracted visual priors from human videos and then repeats and improves them by utilizing a reinforcement learning policy during interaction in the real setting.  

\noindent\textbf{Visual affordance understanding for tasks. }The authors in~\cite{deng20213d} propose a 3D dataset for benchmarking visual affordances with the goal of learning for tasks. However, the challenge of classifying robust affordance categories still remains when undergoing rotations. \cite{xu2022partafford} similarly introduces a learning method for object affordances. Their results indicate that sparse human-like supervision can be used in a natural setting for generalization. In this work, we take a fundamentally different approach where our objective is to exercise the freedom to deviate from the nominal trajectory as long as the task is satisfied, in terms of the human cognitive assessment of the task.   

Our main contributions are (i) exploratory extraction framework of task/motion freedoms and constraints from a single visual demonstration, (ii) user interaction integration into the exploration as feedback, and (iii) enabling generalization to new environments and new agent embodiments while respecting the modeled task's inherent features.

%\url{https://arxiv.org/pdf/2103.16397.pdf} 3D AffordanceNet: A Benchmark for Visual Object Affordance Understanding

%\url{https://arxiv.org/pdf/2202.13519v1.pdf} PartAfford: Part-level Affordance Discovery from 3D Objects
\iffalse
\url{https://github.com/lhc1224/OSAD_Net#-dataset-} PAD and PADv2 datasets

\url{https://users.umiacs.umd.edu/~fer/affordance/part-affordance-dataset/index.html} RGB-D Part Affordance Dataset for tools

\url{https://github.com/enriccorona/YCB_Affordance} Dataset for grasp positions for objects
\fi
%The scientific community has for a long time been interested in a method to teach robots via visual demonstrations. 
}

==> ch5_experiments.tex <==
\section{Experiments} \label{sec:experiments}

\todo{Write the performed experiments!}

\subsection{Skill Detection using Defined Active Checks}

\subsection{Object Unknown Property Inference from Skill Execution Sequence}

\subsection{Restructuring the Concept Hierarchy}


==> definitions/macros.tex <==
%% LyX 2.3.4.2 created this file.  For more info, see http://www.lyx.org/.
%% Do not edit unless you really know what you are doing.
% \documentclass[english,letterpaper, 10 pt, conference]{ieeeconf}
% \usepackage[T1]{fontenc}
% \usepackage[latin9]{inputenc}
% \usepackage{verbatim}
% \usepackage{babel}
% \begin{document}


\global\long\def\vsafe{v_{\text{safe}}}% 
\global\long\def\tsafe{t_{\text{safe}}}% 
\global\long\def\safetycurve{\mathcal{S}_{\text{CG}}}% 



\global\long\def\dualquaternion#1{\underline{\boldsymbol{#1}}}%

\global\long\def\quaternion#1{\boldsymbol{#1}}%

\global\long\def\dq#1{\underline{\boldsymbol{#1}}}%

\global\long\def\quat#1{\boldsymbol{#1}}%

\global\long\def\mymatrix#1{\boldsymbol{#1}}%

\global\long\def\myvec#1{\boldsymbol{#1}}%

\global\long\def\mapvec#1{\boldsymbol{#1}}%

\global\long\def\dualvector#1{\underline{\boldsymbol{#1}}}%

\global\long\def\dual{\varepsilon}%

\global\long\def\dotproduct#1{\langle#1\rangle}%

\global\long\def\norm#1{\left\Vert #1\right\Vert }%

\global\long\def\mydual#1{\underline{#1}}%

\global\long\def\hamilton#1#2{\overset{#1}{\operatorname{\mymatrix H}}\left(#2\right)}%

\global\long\def\hami#1{\overset{#1}{\operatorname{\mymatrix H}}}%

\global\long\def\tplus{\dq{{\cal T}}}%

\global\long\def\getp#1{\operatorname{\mathcal{P}}\left(#1\right)}%

\global\long\def\getd#1{\operatorname{\mathcal{D}}\left(#1\right)}%

\global\long\def\swap#1{\text{swap}\{#1\}}%

\global\long\def\imi{\hat{\imath}}%

\global\long\def\imj{\hat{\jmath}}%

\global\long\def\imk{\hat{k}}%

\global\long\def\real#1{\operatorname{\mathrm{Re}}\left(#1\right)}%

\global\long\def\imag#1{\operatorname{\mathrm{Im}}\left(#1\right)}%

\global\long\def\imvec{\boldsymbol{\imath_{m}}}%

\global\long\def\vector{\operatorname{vec}}%

\global\long\def\mathpzc#1{\fontmathpzc{#1}}%

\global\long\def\cost#1#2{\underset{\text{#2}}{\operatorname{\text{cost}}}\left(\ensuremath{#1}\right)}%

\global\long\def\diag#1{\operatorname{diag}\left(#1\right)}%

\global\long\def\setvector{\mathcal{Q}}%

\global\long\def\dqd#1{\widetilde{\dq{#1}}}%

\global\long\def\vecjoints{\myvec{\Theta}}%

\global\long\def\dqrot#1{\quat r_{#1}}%

\global\long\def\dqpos#1{\quat t_{#1}}%

\global\long\def\mathpzc#1{\fontmathpzc{#1}}%

\global\long\def\cost#1#2{\underset{\text{#2}}{\operatorname{\text{cost}}}\left(\ensuremath{#1}\right)}%

\global\long\def\closedballset{\ensuremath{\mathbb{B}}}%

\global\long\def\complexset{\ensuremath{\mathbb{C}}}%


\global\long\def\realset{\ensuremath{\mathbb{R}}}%


\global\long\def\rationalset{\ensuremath{\mathbb{Q}}}%

\global\long\def\integerset{\ensuremath{\mathbb{Z}}}%

\global\long\def\naturalset{\ensuremath{\mathbb{N}}}%

\global\long\def\SE#1{\ensuremath{SE(#1)}}%

\global\long\def\SO#1{\ensuremath{SO(#1)}}%


\global\long\def\SU#1{\ensuremath{SU(#1)}}%


\global\long\def\liealgebraSE#1{\ensuremath{\mathfrak{se}\left(#1\right)}}%

\global\long\def\liealgebraSO#1{\ensuremath{\mathfrak{so}\left(#1\right)}}%

\global\long\def\liealgebraSU#1{\ensuremath{\mathfrak{su}\left(#1\right)}}%

\global\long\def\dualmatrix#1{\left\llbracket \left\llbracket #1\right\rrbracket \right\rrbracket }%

\global\long\def\quatset{\ensuremath{\mathbb{H}}}%

\global\long\def\unitquatgroup{\ensuremath{\text{Spin}(3)}}%

\global\long\def\unitquatset{\mathcal{S}^{3}}%

\global\long\def\dualquatset{\mathbb{H}\otimes\mathbb{D}}%
 %

\global\long\def\unitdualquatgroup{\text{Spin}(3)\ltimes\mathbb{R}^{3}}%

\global\long\def\unitdualquatset{\dq S}%

\global\long\def\kinerotation{\quat r}%
\global\long\def\kineposition{\quat p}%
 

\global\long\def\errorrotation{\quat e_{o}}%
\global\long\def\errorposition{\quat e_{t}}%
 
% \end{document}


==> definitions/packages2include.tex <==

% \IEEEoverridecommandlockouts                              % This command is only needed if 
                                                          % you want to use the \thanks command

% \overrideIEEEmargins   
\usepackage[utf8]{inputenc}
\usepackage{leftidx}
\usepackage{bm}
\usepackage{amssymb,amsmath,amsfonts,empheq}
\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}%
% \usepackage{amsthm}
\usepackage{graphicx}
\usepackage{siunitx}
\usepackage{multicol}
%% Added for Pseudocode
\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage[noend]{algpseudocode}
% \usepackage{type1cm}
% \usepackage{pifont}% http://ctan.org/pkg/pifont
%\newcommand{\cmark}{\ding{51}}%
%\newcommand{\xmark}{\ding{55}}%
\usepackage{lettrine}
% \usepackage{amsmath} % assumes amsmath package installed
% \usepackage{amssymb} 
\usepackage{color}
\usepackage{cite}
\usepackage{breqn}
\usepackage{tikz}
\usepackage{array}
\usepackage{import}
%\usepackage[latin1]{inputenc}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{optidef}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{siunitx}
%% Added for Pseudocode
\usepackage{algorithm}
\usepackage{multirow}
\usepackage{cite}
\usepackage{import}
\usepackage[draft]{hyperref}
%\usepackage{subcaption}
%\captionsetup{font=small}
\usepackage{microtype}
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{comment}
\setlength{\belowdisplayskip}{3pt} %\setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayskip}{3.5pt} %\setlength{\abovedisplayshortskip}{0pt}
\usepackage{microtype}

\newtheorem{definitn}{Definition}
\newtheorem{prop}{Proposition}
\newtheorem{remrk}{Remark}
\newtheorem{lem}{Lemma}


\usepackage{multirow}


\newcommand{\sclerp}[1]{\text{ScLERP}\left( #1 \right)}

\newcommand{\trans}[1]{\mathfrak T \left( #1 \right)}

